QualityFlow: An Agentic Workflow for Program Synthesis Controlled by LLM Quality Checks

We introduce QualityFlow, a dynamic agentic workflow for program synthesis. Given the English description of a programming problem and a set of unit tests, the model's goal is to synthesize the correct program that solves the problem and passes the tests. QualityFlow includes large language model (LLM) agents resembling a software development team, including code generation, testing, and self-debugging. We propose the LLM Quality Checker, which explicitly "imagines" whether the synthesized programs' execution would conform to the unit tests. The Quality Checks dynamically control the workflow, including actions to submit the final answer, clarify the problem statement, and revert previous workflow steps. Our experiments show that the Quality Checker can precisely accept any correct program, mitigate faulty synthesized tests, and prevent potential workflow deviation. QualityFlow establishes the state-of-the-art results on four program synthesis benchmarks: MBPP, HumanEval, and stricter evaluations from MBPP-EvalPlus and HumanEval-EvalPlus.

==> 1.1.introduction.tex <==





Code generation is a crucial task that has long been a challenge in software development. It plays a vital role in streamlining development processes and enhancing programmer productivity \cite{lu2021codexglue}. Effective code generation techniques can significantly improve efficiency, reduce manual effort, and minimize errors, ultimately leading to faster and more reliable software delivery.%
In a typical code generation scenario, the model's objective is to synthesize code that addresses the problem and passes the provided unit tests, based solely on the natural language descriptions or documentation strings \cite{mbpp,humaneval,apps}.
Large language models (LLMs) have revolutionized the field of zero-shot learning, achieving remarkable results in various tasks, including code generation \cite{ouyang2022training}. However, generating code in a single attempt often proves to be a daunting challenge, failing to fully leverage the potential of these powerful models. As research in LLM-based code generation continues to advance, multi-LLM approaches have emerged as a promising solution, offering trial-and-error opportunities to iteratively refine and enhance the generated output. These approaches harness the same LLM backbones without incurring additional training costs, making them a cost-effective and scalable solution for improving code generation performance.

Reflexion \cite{shinn2024reflexion} and the more recent interactive debate \cite{khan2024debating} are general-domain self-reflection techniques that leverage multiple large language models (LLMs) to iteratively analyze and improve upon previously generated outputs through a process of self-reflection. In the code generation domain, a notable multi-LLM approach is Self-Debugging \cite{chen2023teaching, huang2023agentcoder}, which involves executing the synthesized code against the provided unit tests associated with the problem statement. By running the generated code, identifying failed unit tests, and incorporating the error and trace information, a more comprehensive prompt is created and fed back to the LLM. This iterative process allows the LLM to revise the code, aiming to pass the previously failed tests.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{example-image-a}
    \caption{An example problem from the MBPP code generation benchmark, where the model needs to study the unit tests in-context to generate a program that solves the problem and passes the unit tests. How does the model know that the generated code will pass the unit tests? Existing code generation systems typically make this assumption implicitly. We propose Quality Checker that explicitly reasons about unit test conformity.}
    \label{fig:mbpp}
\end{figure}


Despite their encouraging performance, existing zero-shot generation and self-debugging methods still face important limitations that are difficult to resolve:
\begin{itemize}
    \item \textit{Assumption of visible unit test conformity.} While problem statements often provide unit tests, current code generation methods only implicitly assume that the generated code will pass these tests (Figure \ref{fig:mbpp}). Self-debugging on the visible tests is generally not feasible, as it would violate the benchmark rules by revealing the ground truth solutions (e.g., in MBPP for pass@1 evaluation). Moreover, no existing methods effectively leverage the provided unit tests to enable language models to reflect on whether the generated code will indeed pass these tests.
    \item \textit{Bottleneck of synthesized test quality.} The quality of synthesized tests plays a crucial role in the self-debugging process. If the synthesized tests lack sufficient quality, they could become a bottleneck, hindering the effectiveness of the self-debugging mechanism. Utilizing incorrect tests to debug correct programs may lead to unwarranted errors, and the self-debugger could inadvertently modify a well-functioning program in an attempt to satisfy faulty unit tests (Section [insert relevant section reference]). This situation could result in the introduction of new bugs or unexpected behavior, ultimately defeating the purpose of the self-debugging process.
    \item \textit{Deviation of self-debugging trajectory.} In a multi-step, multi-agent setup, the iterative self-debugging process aims to form a positive trajectory that leads to a correct program. However, if the trajectory deviates from positive improvements, it could become trapped in a loop, reach a fixed point, or degrade further by introducing more bugs and mistakes. Existing multi-agent methods employ static workflows that fail to explore flexible control flows during code generation. As a result, they lack an effective reverting or restarting mechanism to rectify any deviated self-debugging trajectory.
\end{itemize}

Tackling the three limitations mentioned earlier can be achieved through a simple yet effective agentic method. Our key idea is to introduce a Quality Checker agent that examines the correctness of work produced by other Large Language Model (LLM) agents. Unlike existing work that relies on verbal self-reflection methods, our Quality Checker leverages unit tests with Imagined Execution, a technique specifically designed for the code generation domain. The LLM employs Chain-of-Thought (CoT) to think step-by-step and imagine how a synthesized program would execute given the test inputs. It then compares the imagined results with the expected results to determine the correctness of the synthesized code. This approach enables the LLM to explicitly assess visible unit test conformity, validating the otherwise implicit assumption.

Remarkably, we find that Imagined Execution can also be performed when the exact code is not given. By following the problem statement instead of the synthesized code, Imagined Execution can predict the results of a function call, which can be compared with the synthesized results from a unit test synthesizer. Discovering this extrapolated ability, we can also quality-check whether a synthesized test is correct, ensuring that it follows the task specified by the problem statement. This addresses the bottleneck of synthesized test quality and enables self-debugging of the synthesized code.

Furthermore, the Quality Checker is integrated into the code-generation and self-debugging pipeline as a centralized controller agent. It decides the next workflow steps to perform on the intermediate result and rectifies deviations in self-debugging trajectories by restarting or reverting as needed. The Quality Checker transforms the agentic workflow with flexible decision-making abilities, going beyond the static code generation workflows seen in previous work. Quality control is fundamental and indispensable in modern assembly lines, where defective products are discarded or the entire assembly line is stopped when needed. It is perhaps not surprising that the Quality Checker, an important and missing piece in today's code generation pipelines, can address three critical limitations in one method, provided the idea can be executed successfully.

\textit{Will Chain-of-Thought emulation of program execution be correct?} Our findings suggest that Chain-of-Thought (CoT) can sometimes emulate program execution with precision (e.g., when the actual code is provided), while at other times, it may be more prone to hallucination. This hallucination phenomenon is related to, but distinct from, the hallucination observed in other domains, such as natural language processing (NLP). It features algorithmic reasoning pitfalls.

Compared to hallucination in NLP, hallucination in CoT execution emulation can be more easily identified by comparing the Imagined Execution to ground truth execution results and traces. Our paper will dedicate a special case study and share an Algorithmic Reasoning Hallucination dataset (ARH) that highlights CoT execution emulation hallucinations (Section X).

Our central question then becomes: Can we design a high-performance agentic workflow that effectively leverages the imperfect Quality Checker? This is a non-trivial problem. It requires a thorough study of Imagined Execution to overcome the hallucination problem encountered in LLM Chain-of-Thought, as well as a careful design of the agentic workflow with coherent placement of the Quality Checker and all other agents, in order to achieve effective overall performance on the actively-studied code generation problem (Section Y).

















In this paper, we introduce QualityFlow. QualityFlow is an agentic workflow system that introduces a novel approach to code generation, leveraging state-of-the-art techniques. It mimics a software engineering team, where specialized agents collaborate to produce high-quality code. The Code Generator agent drafts the initial program, while the Test Designer agent synthesizes unit tests. The Self-Debugger agent iteratively debugs the program based on error messages from failed unit tests. At the heart of QualityFlow lies the Quality Checker, a controller agent that orchestrates the workflow. It determines whether the intermediate program or synthesized test meets the necessary quality standards. If the program passes the quality check, it is submitted as the final solution. Otherwise, the Quality Checker invokes the appropriate agent to produce the next iteration. Similarly, if a synthesized test passes the quality check, it is used to guide self-debugging; otherwise, it is discarded. The quality checks are performed by large language models (LLMs) using Imagined Execution based on Chain-of-Thought reasoning. The LLM simulates step-by-step execution, comparing the actual output with the expected output. The quality check passes if and only if the outputs match, for both code and test quality checks. If the Quality Checker still rejects the program after self-debugging, it may invoke the Clarifier agent to explain the problem statement and clear up any misunderstandings. The Code Generator is then restarted for one more attempt. However, if the Quality Checker continues to reject the result, it is likely that the workflow trajectory has deviated too far, and all self-debugging and clarification steps are reverted.




























We conduct extensive experimentation on various code generation benchmarks, with a particular emphasis on standard benchmarks like MBPP, where the conformity to visible unit tests is unverified. This allows us to effectively utilize and evaluate our Quality Checker. The results demonstrate that QualityFlow has achieved state-of-the-art performance on benchmarks such as MBPP, MBPP-EvalPus, outperforming existing methods, including single-turn prompting and multi-LLM approaches. To validate the overall design of our agentic workflow, we carry out comprehensive ablation studies. Furthermore, we analyze the Quality Checker in detail, highlighting its ability to navigate the workflow effectively. Particular attention is given to measuring the LLM-emulated execution performance from Imagined Execution.
Our evaluation addresses the following research questions: 
\begin{enumerate}[label=RQ\arabic*, left=6pt]
    \item \textit{Can QualityFlow achieve a new state-of-the-art performance on Python code generation benchmarks?} QualityFlow achieved 93.4\% pass@1 accuracy on MBPP, a new state-of-the-art performance. On ABCDE, QualityFlow achieved new state-of-the-art results, too. 
    
     \item \textit{Can the Code Quality Checker improve the final results by navigating the workflow?}
    We show that our Imagined Execution can accurately predict Python program execution results through Chain-of-Thought, with \jason{numbers}. Performance improvement is how much? 
 
    \item \textit{Can the Test Quality Checker validate LLM-generated tests and enable self-debugging?} Can Chain-of-Thought successfully predict the execution results given program 
    descriptions without the actual code?  
    Majority vote is used. Need experiments.

    
     \item \textit{When will LLM hallucinations occur when emulating program execution?} 
     We conduct a case-study to analyze patterns of LLM hallucination when emulating program execution. Through our experiments, various pitfalls of LLM algorithmic reasoning have been observed, and we introduce a ARH dataset for future analysis.

     
     

    
    

     
\end{enumerate}











The contributions of our paper are summarized as follows:
\begin{itemize}
    \item We introduce QualityFlow an agentic workflow with state-of-the-art performance on various code generation benchmarks, including MBPP. 
    \item We introduce Imagined Execution, a key component of QualityFlow where LLMs predict synthesized program correctness given correct unit tests, to effectively check for unit test conformity of generated code and the correctness of synthesized tests.
    \item We introduce Quality Checker, a centralized controller agent that navigates the agentic workflow and determines the agent to be invoked, taking Imagined Execution as evidence for effective navigation.  
    \item We conduct comprehensive study of our workflow and justify our design decisions. We show  that each of the QualityFlow agents can be measured and developed independently, and each of them is carefully incorporated to improve the overall performance of the workflow.
    \item We share an LLM algorithmic reasoning hallucination (ARH) dataset that includes 1234 data points with incorrect algorithmic reasoning by the LLMs, for future studies of LLM hallucination issues exposed by Chain-of-Thought execution emulation.
\end{itemize}





\jason{For every sentence: is every part of the statement true by the most rigorous standards? Will readers see the same thing as the writers mean to express? Does the paragraph do its job as a component of the paper? Is the writing conceptually easy to understand?}


==> 1.1.introduction_2.tex <==

Large Language Models (LLMs) have achieved remarkable progress in code-related tasks, particularly in the realm of code generation. Their ability to synthesize source code from natural language problem descriptions or docstrings, optionally accompanied by programming context, has been a significant breakthrough. These natural language inputs encompass programming problem statements or function specifications, allowing LLMs to understand the requirements and generate corresponding code snippets or complete programs \cite{mbpp,humaneval,apps}. This capability has opened up new avenues for streamlining software development processes and enhancing programmer productivity.

As Large Language Models (LLMs) for code generation continue to evolve, the approaches have progressed from the initial zero-shot generation to more sophisticated techniques like self-debugging and Reflexion \cite{}, leading to increasingly improved performance.
In zero-shot generation, a single query is made to the LLM, relying solely on the pre-trained model's capabilities for code generation. Most modern foundational models \cite{} are pre-trained on code-related tasks, making this approach effective to a certain extent.
On the other hand, self-debugging involves executing unit tests associated with the problem statement. By running the synthesized code, identifying failed cases, and incorporating error and trace information, a richer prompt is created to query the LLM, allowing it to revise the code with the goal of passing the previously failed tests.
Agentic flow takes it a step further by utilizing multiple LLM agents and introducing more components into the system, typically including a test generator to increase the coverage of unit tests, thus aiding the self-debugger agent in revising the code more effectively.
These advancements in LLM-based code generation techniques have led to increasingly improved performance, leveraging the strengths of pre-trained models while incorporating iterative refinement and collaboration among specialized agents to produce more robust and reliable code solutions.

There are several major issues with the existing LLM code generation methods.
During self-debugging, the usage of visible unit tests are too naive. For datasets with separated of visible and hidden unit tests, e.g., HumanEval, the visible test samples are typically simply executed to gather error or trace information. However, for some samples in the dataset, the provided visible tests are too simple and easy to pass but usually the generated program will fail in executing the hidden tests. While for dataset like MBPP as there are no hidden tests, part of the tests are treated as visible and executed to participate in the self-debugging, which violates the pass@1 requirement. The option of emulating the process of execution of the tests without actually running them which could potentially provide better context for self-debugging hasn't been explored. 
Second, the quality of the test generator could become the bottleneck of the entire system. Incorrect tests could easily push the self-debugger make wrong revisions on the code, in its worst case, it make the originally correct code goes wrong. 
Third, it lacks an effective hard reset mechanism that could be effectively when the initially generated code is very wrong. Mis-understanding the problem description often happens to human developer and also observed in LLMs, with a largely wrong code to start with, even lots of efforts are spent on test generation and self-debugging it might not be able to reach a correct answer. A reset and re-try mechanism should be considered in such situations.  

In this paper, we propose an innovative multi-agent based code generation solution that integrates the concepts of chain-of-thought based code/test quality checking, test synthesis, self-debugging, and problem clarification. The agentic flow consists of 8 agents working together to generate code, synthesize unit tests, perform self-debugging, conduct quality checks, and rephrase the problem statement. One of the main innovations, besides the proposed agentic flow, is the quality checker. It can emulate the problem execution process without actually executing the code, using step-by-step reasoning. This module is essential for generating pass@1 solutions for datasets without separating visible and hidden tests, such as MBPP. It also helps in cases where the visible tests are easy to pass, but the hidden tests are more challenging. Another contribution is the introduction of the clarifier agent. Its purpose is to rephrase the problem statement given the context of repeated failures in self-debugging, which raises reasonable doubts that the initially generated program might have misunderstood the problem statement. In such cases, synthesizing a new program considering all this context could be a better choice than attempting to repair the existing program.

We address the following research questions.
\paragraph{RQ1. Can QualityFlow, a flexible LLM agentic workflow with quality checks, achieve a new state-of-the-art performance on Python code generation benchmarks? }
Preview the results for each research question. Baldur format \cite{first2023baldur}

\paragraph{RQ2. Can a Test Quality Checker agent based on chain-of-thought successfully validate LLM-generated tests given programming specifications? Does a Test Quality Checker improve the overall workflow?}

Majority vote is used. Need experiments.

\paragraph{RQ3. How accurately can LLMs emulate Python program execution results through chain-of-thought?
 Can a Code Quality Checker with emulated execution improve the overall workflow?}

\paragraph{RQ4. Easy to maintain as independent agents, and are design decisions well justified? 
Ablations and alternative workflow designs?}

\paragraph{RQ5. How accurate should the synthesized tests be for successful self-debugging?}

\paragraph{RQ6. Can a Problem Clarifier agent improve the overall Python code generation performance?}

\paragraph{RQ7. Does QualityFlow improve the performance over single-prompt for different LLM backbones?}








==> 1.1.introduction_backup.tex <==






\label{sec:intro}





Code generation has long been a challenge and a crucial task for streamlining software development processes and enhancing programmer productivity \cite{lu2021codexglue}. In a standard code generation setting, given only natural language descriptions or documentation strings accompanied by unit tests, the model's goal is to synthesize code that solves the problem and passes the tests \cite{mbpp,humaneval,apps}. 
\jason{This is an important problem (two sentences)}
\jason{Existing work fails to do what we want. Merge with the three bullet points of limitations below to 1) focus on the problem, and 2) reduce the paragraph significantly. Do not make arguments that are not supported by the results in the paper (e.g. bottleneck of synthesized test quality). Our TQC did not work. Deviation of self-debugging trajectory is also not shown because we did nothing to study the debugging trajectory. We don't need bullet points. Succinct sentences with lots of efforts put into are better than convoluted bullet points.}
\jason{Important, difficult.}
Although zero-shot learning with large language models (LLMs) achieved breakthrough results at the time of its introduction \cite{ouyang2022training}, generating code in a single attempt proves to be challenging and fails to utilize the full potential of LLMs. 
As LLM methods for code generation continue to evolve, multi-LLM approaches emerge to provide trial-and-error opportunities to produce better output, using the same LLM backbones without incurring additional training costs. Reflexion \cite{shinn2024reflexion} and, more recently, interactive debate \cite{khan2024debating} are general-domain self-reflection techniques where multiple LLMs self-reflect on previously generated results and improve iteratively. For multi-LLM methods in the code generation domain, Self-Debugging \cite{chen2023teaching, huang2023agentcoder} involves executing unit tests associated with the problem statement. By running the synthesized code, encountering failed unit tests, and incorporating the error and trace information, a richer prompt is created to query the LLM, allowing it to revise the code with the goal of passing the previously failed tests.



\begin{figure}[t]
    \centering
    \begin{minipage}{0.6\linewidth}
        \textsc{Problem statement: \newline}
        \footnotesize\texttt{Write a Python function to remove the first and last occurrence of a given character from the string.\newline}
        \normalsize	\textsc{Visible unit tests:}
        \begin{lstlisting}[style=mypython]
assert remove_Occ("hello","l") == "heo"
assert remove_Occ("abcda","a") == "bcd"
assert remove_Occ("PHP","P") == "H"\end{lstlisting}
    \end{minipage}
    \caption{An example problem from the MBPP code generation benchmark (No. 11) requires the model to study the unit tests in context to generate a program that solves the problem and passes the unit tests. How does the model know that the generated code will pass the unit tests? Existing code generation systems typically make this assumption implicitly. We propose Quality Checker, which explicitly reasons about unit test conformity.}
    \label{fig:mbpp}
\end{figure}





Despite their encouraging performance, existing zero-shot generation and self-debugging methods still face important limitations that are difficult to resolve: 
\begin{itemize} 
\item \textit{Assumption of visible unit test conformity.} Although unit tests are often provided in the programming problem statements, current code generation methods only \textit{implicitly assume} that the generated code will follow these unit tests (Figure \ref{fig:mbpp}). Self-debugging on the visible tests is often not possible as it violates the benchmark rules by leaking the ground truth (e.g., MBPP, for pass@1 evaluation), and no methods currently exist to better leverage the visible unit tests provided in the problem statement and offer LLMs an opportunity to reflect on whether the code will pass the tests. 
\item \textit{Bottleneck of synthesized test quality.} The quality of synthesized tests could become a bottleneck in the self-debugging process if the synthesized tests are not of sufficient quality. Clearly, using incorrect tests to debug correct programs may lead to unwarranted errors, and the self-debugger may turn a good program into a flawed one merely to satisfy the faulty unit tests. 
\item \textit{Deviation of self-debugging trajectory.} With a multi-step, multi-agent setup, the iterative self-debugging steps may form a positive trajectory that leads to a correct program in the end. However, if the trajectory deviates from positive improvements, it could become stuck in a loop, reach a fixed point, or simply degrade with more bugs and mistakes. Existing multi-agent methods are \textit{static} workflows and fail to explore flexible control flows during code generation; thus, they lack an effective reverting or restarting mechanism to rectify any deviated self-debugging trajectory. 
\end{itemize}





\jason{We want to introduce, not \textit{start to} introduce, our idea of Quality Checker. However, the introduction is verbose. This paragraph will be merged with the ``in this paper'' paragraph. Generally, the reviewers are right that the introduction is too long. Flow into an interesting solution for an interesting, difficult, and challenging problem that deserve investigation. More justifications can be moved to the third paragraph, which continues to sell our paper, optionally. Low-sell the SOTA results on the third paragraph maybe. Problem, solution, merit.}
Surprisingly, these three limitations can be tackled with a simple and effective agentic workflow method. Our key idea is to introduce a \textit{Quality Checker} agent that examines the correctness of the work produced by other LLM agents. It is not merely a verbal self-reflection method seen in existing work \cite{huang2022large,madaan2024self,khan2024debating}, as our Quality Checker leverages the unit tests with \textit{Imagined Execution}, a method specifically designed for the code generation domain. The LLM uses Chain-of-Thought (CoT) to think step-by-step and \textit{imagine} how a synthesized program would execute given the test inputs, comparing the imagined results with the expected results to determine the correctness of the synthesized code. This approach gives the LLM an opportunity to explicitly assess \textit{visible unit test conformity}, validating the otherwise implicit assumption.
The Code Quality Checker prevents self-debugging from being performed on correctly synthesized programs and degrading their quality due to incorrectly synthesized tests, thereby indirectly addressing the \textit{bottleneck of synthesized test quality}. To directly address this issue, we also explore an extrapolated version of the Imagined Execution algorithm for the Test Quality Checker. Remarkably, we find that Imagined Execution can also be performed even when the exact code is not provided. By following not the synthesized code but the problem statement, Imagined Execution can predict the results of a function call, which can then be compared with the synthesized results from a unit test synthesizer. Discovering this extrapolated ability, we conduct an exploratory study to quality-check whether a synthesized test is correct, whether it aligns with the task specified by the problem statement, and whether it can be used to self-debug the synthesized code, with limited success in addressing the \textit{bottleneck of synthesized test quality}.
Lastly, the Quality Checker is integrated into the code-generation and self-debugging pipeline as a centralized controller agent who decides the next workflow steps to perform on the intermediate results and rectifies \textit{deviations of self-debugging trajectories} with restart/revert mechanisms. The Quality Checker transforms the agentic workflow with flexible decision-making abilities beyond the static code generation workflows seen in previous work \cite{chen2024teaching, huang2023agentcoder}. Quality is everything. Quality control is fundamental and indispensable for modern assembly lines that manufacture cars or gloves, discarding defective products or stopping the entire assembly line when needed. It is perhaps not surprising, after all, that Quality Checker, an important and missing piece in today’s code generation pipelines, can address three critical limitations in one method, if the idea can be executed successfully.




















\jason{This paragraph is not necessarily formulaic. Read the NDG and NI paper. But the writing of this paragraph could use some explanations above to explain the design decision as we go. The goal is to satisfy the hunger of the problem.}
In this paper, we introduce QualityFlow, an agentic workflow system with state-of-the-art code generation performance. The agent-based workflow resembles a software engineering team, consisting of a Code Generator agent that drafts the program, a Test Designer agent that synthesizes unit tests, and a Self-Debugger agent that iteratively debugs the program based on error messages from failed unit tests.
At the core of QualityFlow is the Quality Checker, a controller agent that decides whether to invoke the other agents: if an intermediate program passes the quality check, it is submitted as the final solution; otherwise, a selected agent continues to produce the next intermediate program. Similarly, if a synthesized test passes the quality check, it is used to guide self-debugging; otherwise, the synthesized test is discarded.
The quality checks are performed by LLMs using Imagined Execution based on Chain-of-Thought, where the LLM performs step-by-step reasoning to find the execution output and compares it with the expected output: if and only if the two are equal, then the quality check passes for both code and test quality checks.
After self-debugging, if the Quality Checker still does not accept the program, it indicates that the self-debugging trajectory likely failed to reach a good result. In this case, the Quality Checker will invoke a Clarifier agent to explain the problem statement and clarify any misunderstandings before restarting the Code Generator for one more attempt. Finally, if the Quality Checker still rejects the result, it is likely that the workflow trajectory has fatally deviated, and all self-debugging and clarification steps will be reverted.




























\jason{Cut this. Who wants to read these? Focus on the experiments that we conducted, especially after rebuttal. Reformulate the RQ afterwards.}
We perform comprehensive experimentation on various code generation benchmarks, focusing on standard benchmarks (e.g., MBPP) where visible unit test conformity is unverified, and where our Quality Checker can be utilized and evaluated. Results show that QualityFlow has achieved a new state-of-the-art performance on MBPP and MBPP-EvalPlus, outperforming existing methods including single-turn prompting and multi-LLM approaches. Extensive ablation studies are conducted to justify the overall design of our agentic workflow. We analyze the Quality Checker in detail to demonstrate its ability to navigate the workflow, with a focus on measuring the LLM-emulated execution performance from Imagined Execution. Our evaluation addresses the following research questions:



\begin{enumerate}[label=RQ\arabic*, left=6pt]
    \item \textit{Can QualityFlow achieve a new state-of-the-art performance on Python code generation benchmarks?} QualityFlow achieved 94.2\% pass@1 accuracy on MBPP, a new state-of-the-art (SOTA) performance. Under a stricter evaluation from MBPP-EvalPlus, QualityFlow achieved the SOTA performance as well.
    
    \item \textit{Can the Code Quality Checker improve the final results by navigating the workflow?} We demonstrate that our Imagined Execution algorithm can accurately predict Python program execution results through Chain-of-Thought, resulting in a 13.23\% absolute pass@1 improvement on MBPP, thereby achieving a new state-of-the-art performance.
    
 
    \item \textit{Can the Test Quality Checker validate LLM-generated tests and improve the overall results?} As an exploratory study, we extend the Imagined Execution algorithm to perform quality checks on synthesized tests produced by the Test Designer. We find that the Test Quality Checker, in its current design, can successfully improve the precision of the synthesized test suite, but it has limited success in enhancing the overall pass@1 performance of the workflow.
    
    

     
     
    
    

     
\end{enumerate}










\jason{Update these with the rebuttal results. Spend time on this.}
The contributions of our paper are summarized as follows:
\begin{itemize}
    \item We introduce QualityFlow an agentic workflow with state-of-the-art performance on code generation benchmarks including MBPP. 
    \item We introduce Imagined Execution, a key algorithm in QualityFlow where LLMs predict synthesized program correctness given correct unit tests, to effectively check for unit test conformity of generated code and the correctness of synthesized tests.
    \item We introduce Quality Checker, a centralized controller agent that checks the code (or test) quality to navigate the agentic workflow, with self-critique method based on Imagined Execution for the code domain.  
    \item We conduct comprehensive analysis of our workflow and justify our design decisions. We also propose and include an exploratory study on the Test Quality Checker.
\end{itemize}







==> 1.introduction.tex <==
\label{sec:intro}

\begin{figure}[t]
    \centering
    \begin{minipage}{\linewidth}
        \textsc{Problem statement: \newline}
        \footnotesize\texttt{Write a Python function to remove the first and last occurrence of a given character from the string.\newline}
        \normalsize	\textsc{Visible unit tests:}
        \begin{lstlisting}[style=mypython]
assert remove_Occ("hello","l") == "heo"
assert remove_Occ("abcda","a") == "bcd"
assert remove_Occ("PHP","P") == "H"\end{lstlisting}
    \end{minipage}
    \caption{An example problem from the MBPP code generation benchmark (No. 11) requires the model to study the unit tests in context to generate a program that solves the problem and passes the unit tests. How does the model know that the generated code will pass the unit tests? Existing code generation systems typically make this assumption implicitly. We propose Quality Checker, which explicitly reasons about unit test conformity.}
    \label{fig:mbpp}
\end{figure}


Program synthesis is a long-standing goal of software engineering research \cite{manna1971toward, summers1977methodology, pnueli1989synthesis}, with a history dating back to the 1940s and 50s \cite{backus1957fortran}.
In recent years, marked by artificial intelligence and large language model (LLM) approaches \cite{codet5, codegen, incoder, codellama, deepseekcoder, mistral}, program synthesis has moved from research to real-world applications that streamline software development and enhance programmer productivity \cite{lu2021codexglue}.
We study a standard program synthesis setting \cite{mbpp,humaneval,apps}: given the natural language description (documentation) together with some visible unit tests, the model's goal is to generate a program that satisfies the description and passes a set of evaluation tests (possibly the same as the visible tests) (Figure \ref{fig:mbpp}). 
This setting encapsulates the typical software engineering process.
The most competitive program synthesis benchmarks today (e.g. MBPP, HumanEval \cite{mbpp,humaneval,apps}) follow this setting and are incorporated into the standard evaluation suites of almost all LLMs (Table \ref{tab:passatk}), showing the recognition and interests for this problem from both industry and academia.
Like many other generative AI domains, LLMs had dominated other approaches on the program synthesis benchmarks, but the improvements were largely due to scaling up the model size at a prohibitive cost of millions of dollars of computation \cite{kaplan2020scaling, wei2022emergent}.
With new performance gains and no additional training costs, Agentic Workflow has recently been proposed as a way to orchestrate multiple LLM agents that form a team to self-reflect \cite{shinn2024reflexion}, debate \cite{khan2024debating}, and solve the problem together in a collaborative style that can outperform zero-shot LLM program synthesis~\cite{hong2024metagpt}.
Agentic Workflows provide fertile opportunities where we can break out of the dependence on the LLM scaling law for performance improvements and design agents specifically for program synthesis by incorporating ongoing software engineering research, such as self-debugging \cite{chen2024teaching, agentcoder-self-repair} and automatic test generation \cite{chen2024chatunitest, hanford1970automatic}.

In order to design an Agentic Workflow for program synthesis, existing zero-shot generation and self-debugging methods have important limitations to be resolved: 
\begin{itemize}[topsep=1pt]
\item \textit{Assumption of visible unit test conformity.} Current zero-shot generation methods only \textit{implicitly assume} that the generated code will follow the visible unit tests required by the problem statement (Figure \ref{fig:mbpp}).
Self-debugging on the visible tests can violate the benchmark rules by leaking the ground truth (e.g., MBPP), and no methods currently exist to explicitly examine visible unit test conformity through an opportunity for the LLM to reflect on whether the code will pass the tests. 
\item \textit{Bottleneck of synthesized test quality.} Synthesized tests could be executed and any error could provide feedback for self-debugging, but incorrect tests may be misleading. Clearly, using incorrect tests to debug correct programs may raise unwarranted errors, and the self-debugger may turn a good program into a flawed one merely to satisfy the faulty tests or an instruction to indiscriminately debug the program.
\item \textit{Deviation of self-debugging trajectory.} Repeated self-debugging steps should ideally form a positive trajectory that leads to a correct program in the end. However, if the trajectory deviates in the recurrent process, it could become stuck in a loop, reach a fixed point, or simply degrade with more bugs and mistakes. Existing multi-agent methods are \textit{static} workflows and fail to explore flexible control flows during code generation \cite{agentcoder-self-repair}: they lack an effective reverting or restarting mechanism to rectify any deviated self-debugging trajectory.
\end{itemize}

In this paper, we aim to address these limitations and introduce QualityFlow, an Agentic Workflow for program synthesis that resembles a software engineering team with quality assurance at every level. 
QualityFlow includes a Code Generator agent that drafts the program, a Test Designer agent that synthesizes unit tests, and a Self-Debugger agent that iteratively debugs the program based on error messages from failed unit tests.
At the center of QualityFlow, also our key contribution, is the Quality Checker, a controller agent that decides whether to invoke other agents: if an intermediate program passes the quality check, it is submitted as the final solution; otherwise, a selected agent continues to synthesize the next intermediate program.
Quality checks are performed through an LLM self-reflection method specifically designed for code understanding that we call \textit{Imagined Execution}: the LLM performs Chain-of-Thought reasoning (COT) \cite{chain-of-thought} to emulate the execution output and compares it with output asserted by the unit test. If the outputs are equal, then the quality check passes, thereby explicitly examining unit test conformity.
Quality checks can mitigate the adverse impact of incorrectly synthesized tests during self-debugging by detecting incorrect programs.
After self-debugging, if the Quality Checker still does not accept the program, it indicates that the self-debugging trajectory likely failed to reach a good result, and a Clarifier agent will explain the problem statement and clarify any misunderstandings before restarting the Code Generator for one more attempt. 
Finally, if the Quality Checker still rejects, it is likely that the workflow trajectory has fatally deviated, and all self-debugging and clarification steps will be reverted. 
QualityFlow effectively addresses limitations above and achieves the state-of-the-art (SOTA) program synthesis performance on all benchmarks that we evaluate on, including MBPP~\cite{mbpp}, HumanEval \cite{humaneval}, and more extensive evaluations from EvalPlus for both \cite{evalplus}.




 
    

The contributions of our paper are summarized as follows: 
\begin{itemize}[left=10pt,topsep=1pt]
    \item We introduce QualityFlow, an Agentic Workflow with the SOTA program synthesis performances on four benchmarks: MBPP, MBPP-EvalPlus, HumanEval, and HumanEval-EvalPlus.
    \item We introduce Imagined Execution, a self-reflection method tailored for the program synthesis domain where LLMs predict the correctness of synthesized program through emulated execution with Chain-of-Thought reasoning and explicitly checks for unit test conformity.
    \item We introduce Quality Checker, a centralized controller agent that flexibly navigates the agentic workflow, making control flow decisions---including continuing, restarting, or reverting---based on Imagined Execution's predictions of the correctness of intermediate outputs.
    \item We study the bottleneck of synthesized tests and introduce Test Quality Checker, extending quality checks to synthesized tests and filters out poisonous tests, improving the overall workflow performance.
    \item We introduce Diversified Prompting that uses a diverse set of prompts in parallel to maximize the possibility that a correct solution is produced and accepted by the quality checker.
\end{itemize}


==> 2.methods.tex <==
\begin{figure}[t]
    \small\centering
\includegraphics[width=.9\linewidth]{./figures/newdiag3.png}
	\caption{Quality Flow is an agentic workflow for code generation, where a Quality Checker agent assess the quality of the code (or tests) produced by LLM agents for self-reflection based on code-specific emulated execution. In this figure, Program Generator, Self-Debugger, and Problem Clarifier (with restart) produce intermediate programs that are checked by the Quality Checker. If an intermediate program passes the quality check, then it is submitted as the final solution; otherwise, the next agent continues to produce the next intermediate program. \jason{Diversified prompting.}}
	\label{fig:quality-flow}	
\end{figure}


\begin{algorithm}[t]
\caption{QualityFlow \jason{Diversified prompting}}
\label{alg:qf}
\small
\begin{algorithmic}[1]

\State \textbf{Input}: Problem description, visible unit tests
\State \textbf{Output}: A generated program

\State \textbf{Start}

\State GeneratedCode $\gets$ \Call{CodeGenerator}{Problem, VisibleTests} \label{alg:generator}
\State CodeAccept $\gets$ \Call{CodeQualityChecker}{GeneratedCode, Problem, VisibleTests} \label{alg:qc_generator}

\If{CodeAccept}
\State\Return GeneratedCode
\EndIf
\State SynthesizedTests $\gets$ \Call{TestDesigner}{Problem, VisibleTests} \label{alg:test_designer}
\If{Use Test Quality Checker}
    \State FilteredTests $\gets$ \Call{TestQualityChecker}{SynthesizedTests, Problem, VisibleTests} \label{alg:tqc}
\Else
    \State FilteredTests $\gets$ SynthesizedTests
\EndIf

\For{each attempt from 1 to MaxAttempts}
    \State DebuggedCode $\gets$ \Call{SelfDebugger}{GeneratedCode, Problem, FilteredTests} \label{alg:sd}
    \State CodeAccept $\gets$ \Call{CodeQualityChecker}{DebuggedCode, Problem, VisibleTests} \label{alg:qc_sd}
    \If{CodeAccept}
        \State\Return DebuggedCode \label{alg:sd_return}
    \EndIf
\EndFor
\State ClarifiedProblem $\gets$ \Call{ProblemClarifier}{Problem, VisibleTests, DebuggedCode, CodeAccept} \label{alg:clarifier}
\State ClarifiedCode $\gets$ CodeGenerator(ClarifiedProblem, VisibleTests) \label{alg:clarifier_generator}
\State CodeAccept $\gets$ \Call{CodeQualityChecker}{ClarifiedCode, Problem, VisibleTests} \label{alg:qc_clarifier}

\If{CodeAccept}
    \State\Return ClarifiedCode
\Else
    \State\Return GeneratedCode \Comment{Revert} \label{alg:revert}
\EndIf

\State \textbf{End}

\end{algorithmic}
\end{algorithm}

\subsection{QualityFlow Overview}

QualityFlow is illustrated in Figure \ref{fig:quality-flow}, and a pseudo-code is provided in Algorithm \ref{alg:qf}. 
The Program Generator agent (line \ref{alg:generator} of Alg. \ref{alg:qf}) synthesizes an initial program based on the problem statement and the visible tests (example in Figure \ref{fig:mbpp}), and the generated program is fed into the Code Quality Checker agent to predict whether the program is correct (line \ref{alg:qc_generator}). 
If the quality check passes, the program is submitted; otherwise, the workflow directs to the Test Designer agent that synthesizes a number of unit tests (line \ref{alg:test_designer}). 
As an optional component of QualityFlow, the Test Quality Checker agent predicts the correctness of the synthesized tests and filter out the wrong tests (line \ref{alg:tqc}). 
Given the (filtered) synthesized tests, the Self-Debugger agent revises the code over multiple epochs (line \ref{alg:sd}). 
At every epoch, the revised program is fed into the Code Quality Checker agent (line \ref{alg:qc_sd}).
If any program passes the quality check, it is submitted directly. 
Otherwise, the Quality Checker rejects all intermediate programs, and it is likely that the initial understanding of the problem statement was flawed \cite{mu2023clarifygpt}. The workflow needs a ``reset'' to re-interpret the problem from a different viewpoint, and the Problem Clarifier agent will let the Code Generator re-synthesize a program based on a new understanding (line \ref{alg:clarifier} and \ref{alg:clarifier_generator}).
The final quality check decides whether to submit the re-synthesized program from the Clarifier or the initially synthesized program from the Code Generator, which is equivalent to a revert mechanism to prevent a completely deviated workflow trajectory (line~\ref{alg:revert}).
Overall, QualityFlow performs quality checks at every level in order to navigate the workflow, submit any correct intermediate synthesis, and reset potential trajectory deviations.


\subsection{Program Generator} The Program Generator agent starts the workflow (line~\ref{alg:generator}). The LLM generates a program based on the problem statement provided, along with a set of visible unit tests that the generated program should pass.
At this stage, no additional contextual information is available; the only input is the original problem statement itself.

\subsection{Test Designer} 
The Test Designer agent (line \ref{alg:test_designer} of Alg. \ref{alg:qf}) synthesizes test cases for the Self-Debugger.
Following the typical approach \cite{chen2024teaching, huang2023agentcoder}, our Self-Debugging takes feedback from error messages triggered by test case execution. 
However, some benchmarks (e.g. MBPP) prohibit the execution of the visible tests in the original problem statement to prevent label leakage as the evaluation tests are the same, and, for other benchmarks, even when visible tests are available, they are often limited in both quantity (3 tests typically) and coverage.
Thus, synthesizing additional unit tests is necessary, and Test Designer can generate up to 50 synthesized tests in our setting to guide self-debugging. We use 5 Diversified Prompts on the Test Designer and for 10 common case unit tests each, and our experiments show that common case unit tests lead to higher pass@1 accuracy of the overall workflow than corner case unit tests. 

\subsection{Self-Debugger} 
The Self-Debugger agent (line \ref{alg:sd} of Alg. \ref{alg:qf}) iteratively improves a program through automatic debugging by LLMs with the guidance of test execution \cite{agentcoder-self-repair, chen2024teaching}.
The Self-Debugger starts with the original problem statement, an intermediate synthesized program, and the synthesized test cases.
The synthesized tests are executed on the program by a Python interpreter to obtain the error messages of the failed test cases and the actual return values of the program. 
All the information are formatted into a prompt for the language model to generate a revised version of the program, taking into account the failed tests.

Self-debugging is performed through Chain-of-Thought (COT) \cite{chain-of-thought} style reflection, which asks the LLM to analyze step-by-step to reason about why the program fails the test cases and then to offer revisions accordingly, instead of producing a new program directly. 
This iterative process of analyzing failures, reasoning, and revising the program continues until all tests are passed or the maximum number of epochs is reached. 
The Code Quality Checker inspects the revised program at every epoch, and if the quality check passes, the program is submitted as the final output and the entire workflow terminates (line \ref{alg:sd_return} of Alg.~\ref{alg:qf}), which prevents potential trajectory deviation where self-debugging alters a correctly synthesized code later on.
Our Self-Debugger systematically addresses the failed test cases and iteratively improves the program, steering the LLMs to understand the problem context and reason about the program's behavior, leading to more logical and coherent revisions based on execution feedback. 

\subsection{Quality Checker}



    












The (Code) Quality Checker is a controller agent in QualityFlow that examines the quality of the intermediate synthesized programs and use the information to navigate the workflow (line \ref{alg:qc_generator}, \ref{alg:qc_sd}, and \ref{alg:qc_clarifier} of Alg. \ref{alg:qf}). 
The Quality Checker makes critical contributions to the state-of-the-art performance of QualityFlow (e.g. on MBPP, 14\% higher pass@1 accuracy, Figure \ref{fig:cqc_removal}). 

Quality Checker uses \textit{Imagined Execution} to emulate the execution of tests on the synthesized program.
For some benchmarks where the visible tests in the problem statement are the same as the evaluation tests (e.g. MBPP), directly executing the code on these tests causes label leakage and implicitly changes the pass@1 metric to pass@k, where $k$ is the number of times the evaluation tests are run.
Imagined Execution is an innovative approach that emulates the program's execution on test cases without actually running the tests, which allows quality checks under such setting.
For datasets with separate visible and evaluation tests (e.g. HumanEval), the Quality Checker may run the visible tests directly with a Python interpreter instead of Imagined Execution. 
We conduct experiments in both settings, and Imagined Execution is on par with Python execution in overall workflow pass@1 accuracy (HumanEval, Table \ref{tab:sota}).

\paragraph{Imagined Execution}

In Imagined Execution, the large language model performs Chain-of-Thought reasoning \cite{chain-of-thought} to emulate the execution of a synthesized program given a test input.
The Imagined Execution continues step-by-step and reaches the final return value, and if the result is the same as the test case expects, the Code Quality Checker accepts the program.
If there are multiple tests, the Code Quality Checker verifies all of them, and only if all quality checks pass, the program is considered correct. This strategy leads to high precision (98\% on MBPP, Table \ref{tab:cqc}) and the best pass@1 accuracy for the overall workflow. Recall remains high (98\% on MBPP as well, Table \ref{tab:cqc}), and a slight reduction in recall is not detrimental because the workflow has opportunities to produce the correct synthesis as it continues to the next agents.


\paragraph{Test Quality Checker} 

The adoption of test synthesizers has gained popularity in self-debugging-based code generation \cite{agentcoder-self-repair, chen2024teaching}. However, a major limitation with the existing approach is the quality of synthesized tests, i.e. ``the bottleneck of synthesized test quality'' (62\% of synthesized tests are incorrect, Table \ref{tab:tqc}). If the generated tests are low-quality, self-debugging may be misled by the erroneous feedback, and a correctly synthesized program could degrade into an incorrect one. Our experiments  investigate and present evidence of the limited quality of synthesized tests (Table~\ref{tab:tqc}).

To address the bottleneck of synthesized test quality, we design a Test Quality Checker (TQC) agent that extends the idea of quality checks to filter out poisonous (incorrect) or low-quality tests.
Given the problem statement and a synthesized test input, the Test Quality Checker reasons step-by-step to find the output and compare it with the expected output of the test.
If the two outputs match, the synthesized test is accepted and used in self-debugging; otherwise, it is rejected. 
It is important to note that for the Test Quality Checker, the synthesized program is not an input. 
This is because, at this stage, the correctness of the program is in question, and we cannot rely on a potentially problematic program to judge the synthesized tests. 
In experiments, the Test Quality Checker can identify the incorrect tests with around 80\% recall, leading to 0.8\% improvement of the overall pass@1 performance on MBPP (Figure \ref{fig:tqc}).

\subsection{Problem Clarifier} 
The Problem Clarifier agent explains the problem statement. The problem statement can often be under-specified and misunderstood by programmers or LLMs \cite{mu2023clarifygpt}, leading to incorrect program synthesis during the workflow.
In particular, if the initial understanding by the Code Generator is incorrect, the Self-Debugger sees its output and could be biased toward the same incorrect interpretation.
QualityFlow is not static, and quality checks can detect incorrect program after self-debugging and invoke a Problem Clarifier agent that re-interprets the problem statement, so the Code Generator has a second chance of generating the correct program. 
This is akin to a hard \textit{reset} of the workflow. 

The Problem Clarifier not only re-examines the original problem statement but also considers all the contextual information from the test synthesis, test quality check, and self-debugging trajectories. 
The Code Generator has more contextual information this time to understand where the initial misunderstanding of the problem came from and is instructed to produce a different implementation based on the clarified problem statement.

The re-synthesized program after clarification is given to the Quality Checker for the final check, and if it passes, a submission is made; otherwise, the initial code synthesized by the Code Generator is submitted (line~\ref{alg:revert} in Alg.~\ref{alg:qf}).
Conceptually, knowing that our Quality Checker has high recall (98\% after Clarifier, Table \ref{tab:cqc}), if none of the self-debugging and clarification steps could pass the quality check, it is likely that the workflow has fatally deviated, and the workflow \textit{reverts} to the original synthesis with the least potential for cumulative errors or deviation.




\subsection{Diversified Prompting with Quality Checks}
Quality Checker allows us to introduce a technique called Diversified Prompting, which uses multiple prompts with slight variations for each agent in the workflow.
In early analysis of the Code Generator, we find that different prompts can solve different sets of programming problems with partial overlaps. The pass@1 accuracies from different prompts are similar, so prompt engineering or prompt selection is not effective.
Inspired by re-ranker models \cite{collins2005discriminative, hu2022fix} that re-orders generated outputs to select the most relevant result post-hoc, we create a diversified set of prompts to increase the chances for a correct solution to be produced and be accepted by the Quality Checker. For example, instead of a single code generator, we can use multiple (six, for example) code generators in parallel, creating a reasoning structure that parallels Tree-of-Thought \cite{yao2024tree}.

Diversified Prompting can be seen as the opposite of Self-Consistency \cite{wang2023selfconsistency, chen2024universal}.
Self-Consistency uses the same prompt multiple times and use the majority as the final answer, in order to combat non-determinism of LLM generation where different responses are produced \cite{ouyang2024empirical}.
In contrary, the goal of Diversified Prompting is to encourage the differences and diversity of the LLM responses to increase the possibility that a correct solution is generated among the candidates, relying on the assumption that the post-hoc re-ranking or quality check will be highly accurate to pick up the correct solution later.
In this sense, Diversified Prompting can be seen as a new post-hoc prompt optimization and selection method \cite{deng-etal-2022-rlprompt, zhang2023automatic}.
Indeed, as our experiments show, our Quality Checker is highly accurate, and, as a result, Diversified Prompting can greatly improve the overall workflow performance (4\% for MBPP, Figure \ref{fig:cqc_removal}).















==> 3.evaluation.tex <==



\subsection{Experimental Setup}

We evaluate QualityFlow on various code generation benchmarks, using the standard pass@k metric to assess the correctness of the generated code \cite{kulal2019spoc}. For each programming problem, the model generates $k$ programs, and if any of them pass the unit tests, the problem is considered solved. Since there can be multiple functionally equivalent solutions beyond the ``canonical solution'' (the standard solution given in the benchmark), pass@k is deemed a more appropriate metric than exact match (EM) accuracy for evaluating functional correctness \cite{chen2021evaluating}. Specifically, pass@1 measures the percentage of programs that pass all evaluation tests in a single generation attempt.

For Diversified Prompting, the Program Generator uses 6 diversified prompts to produce varied solutions for each programming problem, some of which are the zero-shot program synthesis prompts seen in prior work \cite{austin2021program, agentcoder-self-repair}. The 6 generated programs form parallel progressions of QualityFlow. For each generated program that does not pass the quality check, 3 epochs of self-debugging are performed with a different diversified prompt at each epoch. Afterwards, 3 Clarifier attempts, each with a diversified prompt, are performed on each of the 6 self-debugging results. The temperature parameter of all LLM agents is set to 0, except for the Test Designer, whose temperature is set to 0.1 to encourage diversity in the tests generated. The Test Designer synthesizes tests in batches of 10 tests per query for 5 rounds, with a maximum of 50 tests per program, subject to post-processing. We use Claude as the large language model service provider in this paper due to an exclusive research agreement, and we have verified that our results generalize to other LLMs in external experiments, sometimes with superior performance. In this paper, ``Opus'' refers to Claude Opus-3 LLM, and ``Sonnet'' refers to Claude Sonnet-3.5-v2, the latest LLM model available.



\subsection{Benchmark Selection}

\label{sec:benchmark}





We evaluate on MBPP and HumanEval, together with more extensive evaluation on MBPP-EvalPlus and HumanEval-EvalPlus. QualityFlow is designed for the typical program synthesis setting that produces a program given a problem statement (e.g. program documentation or natural language task specifications) and visible unit tests. The four benchmarks we evaluate on are the most popular and competitive program synthesis benchmarks today, often used to evaluate the most prominent LLMs (Table \ref{tab:passatk}). 

MBPP is a suitable benchmark to highlight the advantage of QualityFlow because Python execution of the visible tests is not allowed, as they are the same as the evaluation tests. 
We can demonstrate the merit of Imagined Execution and the Quality Checker, where the machine learning model \textit{reasons} about program execution instead of actual execution.
Some previous studies \cite{ldb-self-debug, chen2024teaching} partially violated the benchmark by removing and running some evaluation tests during inference time for self-debugging. Removing evaluation tests from the test suites reduces the difficulty of the problem and leads to an unfair comparison with other methods. 




Unlike MBPP, HumanEval \cite{chen2021evaluating} has separate sets of visible tests and evaluation tests for each programming problem, which allows the use of the Python interpreter to predict code correctness during self-debugging. 
Since the evaluation tests are not run, this does not count as a pass@k violation.
This setting is easier because Python interpreter always obtains accurate execution results and does not rely on model-based knowledge obtained from machine learning. 
For a comprehensive evaluation and rigorous comparison with existing methods under the same setting, we include a \textit{relaxed} version of QualityFlow for HumanEval and HumanEval-EvalPlus, where the Quality Checker selects synthesized programs that pass all visible tests by Python execution.


\subsection{RQ1. Can QualityFlow achieve a new state-of-the-art performance on Python code generation benchmarks?}

\begin{table}[t]
\caption{The pass@1 performance at different workflow steps of QualityFlow, on MBPP. The agentic workflow where LLMs collaborate together to create the program consistently outperforms zero-shot program synthesis with a single-turn LLM prompting across all settings, with absolute improvements marked in \textbf{bold}. Statistics for each agent are reported after all Diversified Prompts.}
\label{tab:steps}
\centering
\resizebox{\linewidth}{!}{


\begin{tabular}{lllrrrrrrrr}
\toprule
Benchmark  & LLM  & Version & Single Attempt &  Prog. Gen. & \multicolumn{3}{c}{Self-Debugger} & Clarifier & Final & $\Delta\uparrow$ \\
   \cmidrule(lr){6-8}
       &      &      &        &           & Epoch 1  & Epoch 2  & Epoch 3  &     \\
       \midrule
\multirow{2}{*}{MBPP}          & Sonnet  & Standard &  81.00 &  86.40 &  93.00 &  93.00 &  93.60 &  93.60 &  94.20 &  \textbf{13.20} \\
                               & Opus    & Standard & 76.00 &  80.80 &  85.00 &  85.20 &  84.60 &  86.20 &  87.00 &  \textbf{11.00} \\
                               \midrule
\multirow{2}{20pt}{MBPP-EvalPlus} & Sonnet  & Standard & 78.31 &  79.37 &  79.10 &  79.10 &  79.10 &  79.63 &  79.89 &  \textbf{1.59} \\
                               & Opus    & Standard & 75.40 &  76.46 &  76.46 &  75.93 &  75.93 &  76.46 &  76.72 &   \textbf{1.32} \\
                               \midrule
\multirow{4}{*}{HumanEval}     & Sonnet  & Standard & 96.34 &  96.34 &  97.56 &  96.95 &  96.95 &  97.56 &  97.56 &   \textbf{1.22} \\
                               & Sonnet  & Relaxed &  96.34 &  97.56 &  98.17 &  98.78 &  98.17 &  98.17 &  98.78 &    \textbf{2.44} \\
                               & Opus    & Standard & 82.32 &  84.76 &  87.20 &  86.59 &  87.20 &  86.59 &  86.59 &   \textbf{4.27} \\
                               & Opus    & Relaxed  & 82.32 &  87.20 &  88.41 &  88.41 &  89.02 &  87.80 &  89.02 &  \textbf{6.71} \\
                               \midrule
\multirow{4}{20pt}{HumanEval-EvalPlus} & Sonnet & Standard &  87.20 &  87.80 &  87.80 &  87.80 &  87.80 &  87.80 &  87.80 & \textbf{0.61} \\
                               & Sonnet & Relaxed  & 87.20 &  89.02 &  89.63 &  89.63 &  89.63 &  89.63 &  89.63 &   \textbf{2.44} \\
                               & Opus  & Standard  & 76.22 &  78.05 &  80.49 &  79.27 &  79.88 &  78.66 &  79.27 &   \textbf{3.05} \\
                               & Opus   & Relaxed  & 76.22 &  79.88 &  81.71 &  81.71 &  81.71 &  81.10 &  81.71 &   \textbf{5.49} \\
\bottomrule
\end{tabular}
}
\end{table}



\begin{table}[t]
\caption{The overall pass@1 performance of QualityFlow compared to the prior reported state-of-the-art results on program synthesis benchmarks. In this table, all QualityFlow experiments use the Sonnet LLM backbone. Through a flexible agentic workflow with quality checks, QualityFlow has established the state-of-the-art (SOTA) results on all benchmarks (emphasized in bold), with improvements over prior SOTA results marked in column $\Delta \uparrow$.}
    \label{tab:sota}
    \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lrrrlrr}
\toprule
Benchmark                 & \multicolumn{2}{c}{QualityFlow}                                 & Single Attempt  & \multicolumn{2}{c}{Prior Published SOTA}        & $\Delta \uparrow$\\
\cmidrule(lr){2-3}\cmidrule(lr){4-4}\cmidrule(lr){5-6}
                                 & Standard                     & Relaxed          & Result          & Method                               & Result   \\
\midrule               
MBPP                          & \textbf{94.2}   &  (not allowed)    & 92.2 & DeepSeek-Coder-V2-Instruct\cite{deepseekcoder}           & 89.4      & 4.8\\
MBPP-EvalPlus                  & \textbf{79.9}  &  (not allowed)    & 78.3  & DeepSeek-Coder-V2-Instruct\cite{deepseekcoder}           & 76.2      & 3.7\\
HumanEval                    & 97.6             & \textbf{98.8}     & 96.3  & LDB\cite{ldb-self-debug}                                 & 98.2      & 0.6 \\
HumanEval-EvalPlus            & 87.8   & \textbf{89.6}    & 87.2  & Instruct-Turbo\cite{evalplus}               &  86.6     & 3.0  \\
\bottomrule
\end{tabular}
}
\end{table}








We evaluate QualityFlow's program synthesis performance on MBPP \cite{austin2021program}, MBPP-EvalPlus \cite{liu2024your}, HumanEval \cite{chen2021evaluating}, and HumanEval-EvalPlus benchmarks \cite{liu2024your}. 
The step-by-step performance breakdown is in Table \ref{tab:steps}. 
The Test Quality Checker is not used and will be explored later in Section \ref{sec:tqc}.
MBPP does not allow execution of the visible tests (relaxed setting), discussed in Sec. \ref{sec:benchmark}.

We observe a consistent increase in pass@1 performance as the workflow progresses through the steps. The Program Generator's performance is equivalent to that of a zero-shot generation method with a single LLM prompt. 
As the workflow advances, multiple LLMs collaborate to improve the initial code generated by the Code Generator, leading to an increased pass@1 metric across all settings (column $\Delta \uparrow$ in Table \ref{tab:steps}), across different LLM backbones and benchmarks.
Compared to single-turn prompting of LLMs, our agentic workflow can uncover the programming potential of LLMs without additional training.

\begin{table}[t]
\caption{The pass@k performance on MBPP of QualityFlow compared to previously reported results. QualityFlow achieves a new state-of-the-art performance on MBPP. Different methods vary the number of generated programs submitted for evaluation (parameter $k$ in pass@k), and we use ``-'' to indicate pass@k results that are not reported for the model.
\jason{considering expanding to humaneval, we need to include additional baselines, after arxiv}
}
\label{tab:passatk}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llllll}
\toprule
                                         & \# of prompts &  pass@1        & pass@5          & pass@10     & pass@100 \\
\midrule
\textbf{QualityFlow (ours)}            & Multiple       & \textbf{94.2} & \textbf{96.2}        &   -      &    -      \\
AgentCoder (2024) \cite{huang2023agentcoder}            & Multiple       &   -            & <=91.8 &      -   &      -    \\
DeepSeek-Coder-V2-Instruct (2024) \cite{deepseekcoder}       & One   & 89.4    & -   &  -  & - \\ 
Claude Sonnet-3.5 (2024, reproduced)     & One   & 88.7          &     -            &    -     &     -     \\
Claude Opus-3 (2024)                     & One   & 86.4          &     -            &    -     &     -     \\
MapCoder (2024)    \cite{islam-etal-2024-mapcoder}                       & Multiple       & 83.1          &     -            &    -     &    -      \\
Reflexion (2023) \cite{shinn2024reflexion}                        & Multiple       &  77.1 & - & - & - \\ 
Self-Debugging, +Trace (2024) \cite{chen2024teaching}          & Multiple       & 76.4  & - & - & - \\
LDB (2024) \cite{ldb-self-debug} & Multiple & 76.0 & - &- \\
Code Llama (2023)\cite{roziere2023code}                        & One   & 62.4          &   -              & 81.1    & 91.9     \\
Code Llama - Python (2023) \cite{roziere2023code}              & One   & 65.6          &     -            & 81.5    & 91.9     \\
Llama 2 (2023) \cite{touvron2023llama}                           & One   & 45.4          &     -            & 66.2    & 83.1    \\
\bottomrule
\end{tabular}
}
\end{table}



We compare the performance of QualityFlow with previously reported state-of-the-art (SOTA) results in Table \ref{tab:sota}. QualityFlow has achieved new state-of-the-art performances on all benchmarks.
QualityFlow achieved this performance because of careful and accurate quality checks throughout the workflow, which explicitly examines visible unit test conformity, rejects incorrect self-debugging programs misguided by erroneous synthesized tests, and navigate the control flow to rectify deviations of workflow trajectory. Quality checks are analyzed further in the following Section \ref{sec:cqc_results}.


MBPP provides a suitable setting to show the advantage of the Code Quality Checker and Imagined Execution, as the visible tests cannot be executed, and QualityFlow achieves the state-of-the-art performance of 94.2\% pass@1 accuracy, a 4.8\% increase over the prior SOTA. 
HumanEval allows a relaxed setting where QualityFlow uses a Python interpreter that replaces the Code Quality Checker, and QualityFlow achieved 98.8\% pass@1, a 0.6\% improvement over the prior SOTA. 
With a stricter evaluation from EvalPlus, QualityFlow also outperformed prior SOTA (86.6\%) with both Imagined Execution Quality Checker (89.6\%) and Python Checker (87.8\%).


We report the pass@k performance of QualityFlow and compare it with prior MBPP results in Table \ref{tab:passatk}. In QualityFlow, with 3 epochs of self-debugging, a maximum of 7 distinct outputs can be produced in total, including intermediate outputs and the final output.
For pass@5 evaluation, we use the first 5 intermediate outputs produced for each synthesized program, in the order of workflow steps without additional reordering. 
Note that in this setting, the Code Quality Checker is not required, as any intermediate output is directly submitted for pass@k evaluation. 
Additionally, not every program goes through all steps of the workflow. For example, self-debugging may terminate early if no synthesized tests are triggered. Thus, pass@k evaluates results from a mixture of workflow steps in QualityFlow.
We observe that the pass@5 performance of QualityFlow exceeds all results shown in Table \ref{tab:passatk}, including pass@100 results from Llama models, demonstrating QualityFlow's effectiveness and efficiency in settings where multiple generated programs are allowed.












\subsection{RQ2. Can the Code Quality Checker improve the final results by navigating the workflow?}

\label{sec:cqc_results}







\begin{table}[t]
\caption{The Code Quality Checker's confusion matrix statistics at different workflow steps of QualityFlow. A positive solution is one that correctly solves the problem. The Code Quality Checker with Imagined Execution is highly accurate.}
\label{tab:cqc}
\resizebox{\linewidth}{!}{
\begin{tabular}{cclrrrrrrr}
\toprule
          Benchmark                  &        LLM                   & Statistic    & Single Attempt       & Prog. Gen. & \multicolumn{3}{c}{Self-Debug} & Clarifier  & Final \\
     \cmidrule(lr){6-8}              &                              &              &      &         & Epoch 1  & Epoch 2  & Epoch 3  &   & \\
     \midrule
\multirow{10}{*}{MBPP} & \multirow{5}{*}{Sonnet} &      Actual positive &  81.00 &  86.40 &  93.00 &  93.00 &  93.60 &  93.60 &  94.20 \\
                     &                      &             Accuracy &  93.20 &  95.40 &  97.20 &  97.40 &  96.60 &  96.80 &  96.20 \\
                     &                      &            Precision &  98.94 &  98.81 &  98.49 &  98.50 &  98.29 &  97.68 &  97.68 \\
                     &                      &               Recall &  92.59 &  95.83 &  98.49 &  98.71 &  98.08 &  98.93 &  98.30 \\
                     &                      &    \% of final output &  75.80 &  83.80 &  93.00 &  93.20 &  93.40 &  94.80 &  94.80 \\
                     \cmidrule(lr){2-10}
                     & \multirow{5}{*}{Opus}&      Actual positive &  76.00 &  80.80 &  85.00 &  85.20 &  84.60 &  86.20 &  87.00 \\
                     &                      &             Accuracy &  87.20 &  92.60 &  94.60 &  94.40 &  95.00 &  95.00 &  94.20 \\
                     &                      &            Precision &  98.47 &  97.91 &  95.23 &  95.23 &  95.23 &  95.11 &  95.11 \\
                     &                      &               Recall &  84.47 &  92.82 &  98.59 &  98.36 &  99.05 &  99.30 &  98.39 \\
                     &                      &    \% of final output &  65.20 &  76.60 &  88.00 &  88.00 &  88.00 &  90.00 &  90.00 \\
                     \midrule
\multirow{10}{50pt}{HumanEval-EvalPlus} & \multirow{5}{*}{Sonnet} &      Actual positive &  95.73 &  96.34 &  97.56 &  96.95 &  96.95 &  97.56 &  97.56 \\
                     &                      &             Accuracy &  93.90 &  96.34 &  96.95 &  97.56 &  97.56 &  96.95 &  96.95 \\
                     &                      &            Precision &  98.04 &  97.50 &  97.55 &  97.55 &  97.55 &  97.55 &  97.55 \\
                     &                      &               Recall &  95.54 &  98.73 &  99.38 & 100.00 & 100.00 &  99.38 &  99.38 \\
                     &                      &    \% of final output &  93.29 &  97.56 &  99.39 &  99.39 &  99.39 &  99.39 &  99.39 \\
                  \cmidrule(lr){2-10}
                     & \multirow{5}{*}{Opus} &      Actual positive &  89.63 &  92.07 &  95.12 &  93.90 &  95.12 &  94.51 &  95.12 \\
                     &                      &             Accuracy &  82.93 &  92.07 &  92.68 &  93.90 &  93.29 &  93.29 &  92.68 \\
                     &                      &            Precision &  96.85 &  96.00 &  95.57 &  95.57 &  95.60 &  95.00 &  95.00 \\
                     &                      &               Recall &  83.67 &  95.36 &  96.79 &  98.05 &  97.44 &  98.06 &  97.44 \\
                     &                      &    \% of final output &  77.44 &  91.46 &  96.34 &  96.34 &  96.95 &  97.56 &  97.56 \\
         \bottomrule
\end{tabular}
}
\end{table}







\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/code_checker_ablations.png}
    \caption{The pass@1 accuracy versus the workflow steps for the standard QualityFlow and the QualityFlow without Code Quality Checker (CQC) (Sonnet LLM). 
    The CQC improves the overall pass@1 performance of the workflow, and each workflow step has a better performance. 
    Without CQC, self-debugging is performed indiscriminately on all intermediate programs. %
    Correct programs will be incorrectly changed, often guided by incorrectly synthesized tests, causing a drastic drop in performance at the Self-Debug epoch 1, which reflect limitations seen in existing work that we call the `` bottleneck of synthesized test quality'' and the ``deviation of self-debugging trajectory''. 
    Note that Diversified Prompting requires the CQC.
    }
    \label{fig:cqc_removal}
\end{figure}







Code Quality Checker (CQC) is an LLM agent that uses Imagined Execution, a Chain-of-Thought process, to evaluate the correctness of synthesized programs by emulating their execution and comparing the results to expected outcomes from unit tests. The LLM's algorithmic reasoning ability is essential for accurately emulating program execution and navigating the QualityFlow.


The Code Quality Checker can be independently assessed as a binary classifier. A synthesized program is considered correct if it passes the evaluation tests, and the CQC's objective is to correctly classify them. 
The accuracy and other confusion matrix statistics of Code Quality Checker with Imagined Execution are presented in Table \ref{tab:cqc}. 



We see from Table \ref{tab:cqc} that the precision of the quality check is high (e.g. 98.81\% on the programs produced by Program Generator on MBPP with Sonnet LLM). 
The high precision is due to our design decision for a stricter quality check, where all Imagined Execution results given the visible test suite need to be as expected in order to accept a synthesized program.
This allows the CQC to carefully select correctly synthesized programs and pass the uncertain ones to further processing in the rest of the pipeline. 
Shown on the row ``\% of final output'' in Table \ref{tab:cqc}, as the agentic workflow continues, more and more programs are accepted by the Code Quality Checker and submitted.
High accuracy, precision, and recall confirm the effectiveness of our carefully designed Code Quality Checker in classifying the correctness of synthesized programs.


Studying the Code Quality Checker this component in isolation is insufficient, as it needs to integrate with the rest of the agentic workflow and improve the overall pass@1 performance. We conducted ablation experiments where the CQC is removed from QualityFlow to find the difference in the pass@1 accuracy. 
When the CQC is removed, there will be no termination condition for the workflow, and every problem will go through all workflow steps for pass@1 evaluation. This is a limitation seen in existing work \cite{huang2023agentcoder}, and we run this variation of QualityFlow to compare with the standard QualityFlow. Figure \ref{fig:cqc_removal} plots the pass@1 accuracy of all workflow steps with and without Code Quality Checker, on MBPP benchmark with Sonnet LLM.

From Figure \ref{fig:cqc_removal}, we see that for the standard QualityFlow with the CQC, the pass@1 accuracy at every step after Code Generator is higher than that without the CQC. The final pass@1 accuracy of the standard setting is 94.2\% on MBPP, higher than 80.2\% without the Code Quality Checker, improving by 14\%.
Without the CQC, all steps in the the workflow will be performed on every program, and correct programs could be incorrectly changed to buggy programs during self-debugging, potentially guided by incorrectly synthesized tests (Table \ref{tab:tqc}). 
This explains a drastic drop in pass@1 accuracy without the CQC at the Self-Debug epoch 1, from 93\% to 56.8\% on MBPP and from 98.17\% to 79.88\% on HumanEval, reflecting limitations seen in existing work that we call the ``bottleneck of synthesized test quality'' and the ``deviation of self-debugging trajectory'' in Introduction.
The CQC can address these two issues by identifying correctly synthesized programs and submit them directly, preventing possible deviation later, and when the self-debugger is misled by incorrect tests, the CQC can identify incorrect programs and invoke the next agent to fix them, restart the workflow, or revert to the initial solution.
Results conclude that the Code Quality Checker plays a central role in navigating the QualityFlow and can bring clear improvements on the overall performance.




\begin{table}[t]
    \caption{Imagined Execution versus a simple baseline LLM method to directly classify program correctness directly for Code Quality Checking on MBPP and HumanEval (single-attempt zero-shot programs). The baseline model tends to be overly optimistic and accept incorrect programs, reflected by a lower specificity than Imagined Execution, and it does not improve the workflow performance beyond single-attempt zero-shot synthesis. Imagined Execution is a critical factor behind QualityFlow's state-of-the-art performance. }
    \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llrrrrrr}
\toprule
Benchmark & Code Quality Checker & Actual Positive & Predicted Positive & Accuracy & Sensitivity & Specificity & Workflow pass@1 \\
\midrule
\multirow{2}{*}{MBPP}      & Simple Yes/No Classifier      &  81.00 &  91.00 &  76.80 &  91.85 &  12.63 & 78.80  \\
                           & Standard Imagined Execution  &  81.00 &  75.80 &  93.20 &  92.59 &  95.79 &  94.20\\
                           \midrule
\multirow{3}{*}{HumanEval} & Simple Yes/No Classifier      &  95.73 &  95.12 &  92.07 &  95.54 &  14.29 & 95.73  \\
                           & Standard Imagined Execution  &  95.73 &  93.90 &  93.29 &  95.54 &  42.86 &  97.56\\
                           & Relaxed Python checker        &  95.73 &  95.73 & 100.00 & 100.00 & 100.00 & 98.78  \\
\bottomrule
\end{tabular}
}
    \label{tab:imagined}
\end{table}


\paragraph{Imagined Execution versus a simple Yes/No LLM critic.} Without Imagined Execution to emulate program execution and check for unit test conformity, the Code Quality Checker would not be as accurate and would not lead to SOTA workflow performance. We implement a simple baseline that replaces Imagined Execution with an LLM that directly predicts whether the code is correct as a binary classifier. The results are in Table \ref{tab:imagined}.
Our experiments show that the baseline method is overly optimistic that tend to predict that the synthesized programs are correct, shown by the lower specificity than Imagined Execution, along with lower accuracy.
When code quality checking is done with this simple critic, QualityFlow performance can be lower than single-attempt zero-shot program synthesis on MBPP, dropping from 81.0\% to 78.8\%, and equal on HumanEval with 95.73\%.
Indeed, the method for code quality checking is critical for the success of QualityFlow, and using Python interpreter to execute the visible tests to check code creates a perfect classifier and the best QualityFlow performance on HumanEval.

\subsection{RQ3. Can the Test Quality Checker validate LLM-generated tests to improve self-debugging and overall results?}






\begin{table}[t]
\caption{The Test Quality Checker's (TQC's) performance to select incorrect LLM-designed tests. The TQC is performed on the more challenging MBPP and MBPP-EvalPlus problems for which the code generator's program did not pass the Code Quality Checker, and on the triggered synthesized tests for which the code generator's program did not pass. 
The TQC can identify the incorrect tests with recall higher than the background percentage of incorrect tests, thereby preventing incorrect tests from misleading the Self-Debugger. A positive test is one that is incorrect.}
\label{fig:tqc}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lrrrrrrrr}
\toprule
Benchmark    & \multicolumn{2}{c}{MBPP}  & \multicolumn{2}{c}{MBPP-EvalPlus} & \multicolumn{2}{c}{HumanEval}  & \multicolumn{2}{c}{HumanEval-EvalPlus}  \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
LLM                                 & Sonnet & Opus & Sonnet & Opus & Sonnet & Opus & Sonnet & Opus \\
\midrule
                                    Total programs & 500 & 500 & 378 & 378 & 164 & 164 & 164 & 164 \\
                            Total covered programs & 81 & 117 & 27 & 44 & 4 & 14 & 4 & 14 \\
                                       Total tests & 3992 & 5830 & 1313 & 2188 & 190 & 701 & 190 & 701 \\
                             Total triggered tests & 1963 & 3196 & 502 & 1072 & 39 & 305 & 39 & 305 \\
    Avg. incorrect and triggered tests per problem &  15.67 &  19.63 &  14.91 &  17.12 &   4.25 &   9.71 &   4.25 &   9.64 \\
       Percentage of incorrect and triggered tests &  62.25 &  70.62 &  68.33 &  65.49 &  43.59 &  44.59 &  43.59 &  44.26 \\
       \cmidrule(lr){1-1}\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                      Accuracy &  55.17 &  70.81 &  61.16 &  70.34 &  46.15 &  84.92 &  46.15 &  84.59 \\
                     Precision &  60.74 &  74.20 &  68.23 &  71.92 &  41.67 &  75.86 &  41.67 &  75.29 \\
                        Recall &  79.13 &  89.94 &  80.76 &  89.74 &  58.82 &  97.06 &  58.82 &  97.04 \\
                            F1 &   0.69 &   0.81 &   0.74 &   0.80 &   0.49 &   0.85 &   0.49 &   0.85 \\
        \cmidrule(lr){1-1}\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
                    Total incorrect tests filtered & 967 & 2030 & 277 & 630 & 10 & 132 & 10 & 131 \\
                 Covered programs before filtering & 78 & 115 & 23 & 41 & 4 & 14 & 4 & 14 \\
                  Covered programs after filtering & 44 & 59 & 13 & 21 & 3 & 10 & 3 & 10 \\
 Avg. triggered tests per problem before filtering &  25.17 &  27.79 &  21.83 &  26.15 &   9.75 &  21.79 &   9.75 &  21.79 \\
Avg. incorrect and triggered tests per problem before filtering &  15.67 &  19.63 &  14.91 &  17.12 &   4.25 &   9.71 &   4.25 &   9.64 \\
  Avg. triggered tests per problem after filtering &   8.43 &   7.80 &   7.38 &   9.33 &   5.00 &  13.10 &   5.00 &  13.10 \\
Avg. incorrect and triggered tests per problem after filtering &   5.80 &   3.85 &   5.08 &   3.43 &   2.33 &   0.40 &   2.33 &   0.40 \\
\bottomrule
\end{tabular}

}
\end{table}




\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/test_checker_ablations.png}
    \caption{The pass@1 performance of QualityFlow when the Test Quality Checker (TQC) is removed. Test Quality Checker improves the overall performance by 1\% on MBPP compared to the standard setting. On HumanEval, removing TQC also causes self-debugging performance to drop, but the drop is rectified by Clarifier later in the workflow.}
    \label{fig:tqc}
\end{figure}






\renewcommand{\arraystretch}{1.05} 
\begin{table}[t]
    \centering
\caption{The overall pass@1 performance when the Test Quality Checker (TQC) is removed from the workflow, compared to the standard QualityFlow. The TQC often improves the overall performance when the better LLM (Sonnet) is used, but it often has negative effect when the weaker LLM is used (Opus), which reflects that the test quality checking problem a more challenging task than code quality checking. 
}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{lllrrr}
\toprule
LLM & Benchmark & Setting & Standard QualityFlow & QualityFlow without TQC & Delta \\
\midrule
\multirow{6}{*}{Sonnet} & MBPP                                   & Standard &  94.20 &  93.40 &   0.80 \\
                        \cmidrule(lr){2-6}
                        & MBPP-EvalPlus                          & Standard &  79.89 &  79.89 &   0.00 \\
                        \cmidrule(lr){2-6}
                        & \multirow{2}{*}{HumanEval}             & Standard &  97.56 &  96.95 &   0.61 \\
                        &                                        & Relaxed &  98.78 &  98.17 &   0.61 \\
                        \cmidrule(lr){2-6}
                        & \multirow{2}{40pt}{HumanEval-EvalPlus} & Standard &  87.80 &  88.41 &  -0.61 \\
                        &                                        & Relaxed &  89.63 &  89.63 &   0.00 \\
                        \midrule
\multirow{6}{*}{Opus}   & MBPP                                   & Standard &  87.00 &  86.60 &   0.40 \\
                        \cmidrule(lr){2-6}
                        & MBPP-EvalPlus                          & Standard &  76.72 &  77.25 &  -0.53 \\
                        \cmidrule(lr){2-6}
                        & \multirow{2}{*}{HumanEval}             & Standard &  86.59 &  87.20 &  -0.61 \\
                        &                                        & Relaxed &  89.02 &  90.24 &  -1.22 \\
                        \cmidrule(lr){2-6}
                        & \multirow{2}{40pt}{HumanEval-EvalPlus} & Standard &  79.27 &  80.49 &  -1.22 \\
                        &                                        & Relaxed &  81.71 &  82.93 &  -1.22 \\
\bottomrule
\end{tabular}
}
    \label{tab:tqc}
\end{table}
\renewcommand{\arraystretch}{1}

\label{sec:tqc}

We study further on the bottleneck of synthesized test quality and propose Test Quality Checker (TQC) to extend idea of quality checks toward selection of synthesized tests.
The TQC's goal is to predict the correctness of synthesized tests. 
As the synthesized code may not be correct, the TQC predicts the result of a unit test solely based on the problem statement. This contrasts with Imagined Execution in Code Quality Checker, which is provided with both the problem statement and the synthesized code. 
One should reasonably expect a degradation of the emulation execution under such constraints.
Note that while Test Quality Checker has limited effectiveness in addressing the bottleneck of synthesized tests quality, the Code Quality Checker can also detect incorrect programs post-hoc from self-debugging .

The performance of the Test Quality Checker can also be evaluated independently as a classifier, based on whether it can classify that a synthesized test is correct or incorrect. 
A synthesized test is considered correct if the canonical program, which is the ground truth solution, passes the test. 
The accuracy and other confusion matrix statistics are presented in Table \ref{fig:tqc}, for the programs that did not pass the Code Quality Checker, and for synthesized tests that are triggered on the synthesized code that could potentially provide self-debugging feedback.
This subset of the problems are more challenging, as the Code Quality Checker is an accurate model (Table \ref{tab:cqc}), and that the Program Generator's solution did not pass the quality check. 
This subset of tests are also more challenging, because trivial tests that are easy to pass will not be triggered.
These two factors are unavoidable and set forth significant challenges to the TQC's classification objective.

In Table \ref{fig:tqc}, we see 62.25\% synthesized tests for self-debugging are incorrect on MBPP with Sonnet LLM, which proves the bottleneck of synthesized test quality. 
The Test Quality Checker can successfully recall and filter out 79.13\% of the synthesized tests are incorrect, preventing these faulty tests from misguiding the Self-Debugger. 

We conduct experiments with the TQC integrated into QualityFlow and measure the change in the overall pass@1 performance. The experiments are conducted on all benchmarks, with both Claude Sonnet and Opus LLMs.
The results are reported in Table \ref{tab:tqc}. 

Integrating the Test Quality Checker into QualityFlow can often lead to positive improvements on the overall pass@1 accuracy when the better LLM (Sonnet) is used, which contributes to the state-of-the-art performance of QualityFlow for both MBPP and HumanEval, by 0.8\% and 0.61\% respectively. However, when the weaker LLM (Opus) is used, the performance usually drops, which reflects that the test quality checking problem a more challenging task than code quality checking.
As language models gain in size and capabilities, the quantitative scaling can lead to emergence of new qualitative abilities \cite{wei2022emergent}, and test quality checking is one of such emerging methods enabled by the latest LLMs. 
While the Test Quality Checker has high recall and contributes to the workflow's state-of-the-art performance, it has not yet perfectly addressed the bottleneck of synthesized test quality, as its recall is 80\%, compared to the Code Quality Checker's 98\% recall. Better test quality checking methods to better utilize synthesized tests for self-debugging and program synthesis in future research. 
























\subsection{Ablation experiments and further analysis}

We conduct extensive ablation experiments and analysis on QualityFlow to justify the design decisions. Our findings are summarized here, and further details are in the Appendix.




\begin{table}[t]
\caption{We experiment with DeepSeek LLM backbone, and we see that QualityFlow outperforms single-attempt LLM prediction. DeepSeek-v2.5 underperforms Claude Sonnet across all settings, and our work uses Claude Sonnet as the default QualityFlow LLM backbone.}
\label{tab:deepseek}
    \centering
    \resizebox{0.76\linewidth}{!}{
    \begin{tabular}{lllrr}
\toprule
Dataset & Setting& LLM & Single Attempt & QualityFlow pass@1 \\
\midrule
\multirow{3}{*}{MBPP}      & \multirow{3}{*}{Standard} & Deepseek &  79.80 &  87.80 \\
                           &                           & Opus &  80.80 &  87.00 \\
                           &                           & Sonnet &  86.40 &  \textbf{94.20} \\
                                                      \midrule
\multirow{6}{*}{Humaneval} & \multirow{3}{*}{Standard} & Deepseek &  92.68 &  93.90 \\
                           &                           & Opus &  84.76 &  86.59 \\
                           &                           & Sonnet &  96.34 &  \textbf{97.56} \\
                                                      \cmidrule(lr){2-5}
                           & \multirow{3}{*}{Relaxed}  & Deepseek &  92.68 &  96.95 \\
                           &                           & Opus &  87.20 &  89.02 \\
                           &                           & Sonnet &  97.56 &  \textbf{98.78} \\
\bottomrule
    \end{tabular}
}
\end{table}


\paragraph{DeepSeek integration with QualityFlow} DeepSeek \cite{deepseekcoder} was the prior SOTA method on MBPP with 89.4\% pass@1 (Table \ref{tab:sota}). It is a LLM and a single-attempt zero-shot program synthesis method. We implemented QualityFlow with the DeepSeek LLM backbone, and the workflow continues to perform better than zero-shot synthesis in all settings. The standard QualityFlow with Sonnet LLM has superior performance than DeepSeek QualityFlow.

\paragraph{LDB reproduction with Sonnet LLM} LDB \cite{ldb-self-debug} was the prior SOTA method on HumanEval with 95.1\% pass@1 using the Reflexion LLM backbone \cite{shinn2024reflexion}. To eliminate the confounding effect of different LLMs and compare the program synthesis methods fairly, we reproduced LDB with Sonnet LLM, and LDB also has 95.1\% pass@1, lower than 98.8\% in the authors' original setting (Table \ref{tab:sota}). With the same Sonnet LLM, QualityFlow achieves 98.8\% pass@1 on HumanEval (Table \ref{tab:sota}), proving that the performance advantage comes from our workflow design, not the LLMs used.




\begin{table}[t]
\caption{We conduct ablation experiments that remove Clarifier and Revert separately and measure the overall pass@1 of the entire workflow (Sonnet LLM). Removing each component causes performance drop, and the standard QualityFlow has consistently the best performance.}
\label{tab:removal}
\centering
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{lllr}
\toprule
Dataset & Setting & Ablation & QualityFlow pass@1 \\
\midrule
\multirow{3}{*}{MBPP}      & \multirow{3}{*}{Standard}   & Standard &  \textbf{94.20} \\
                           &                             & Remove Revert &  93.60 \\
                           &                             & Remove Clarifier &  93.80 \\
\midrule
\multirow{6}{*}{HumanEval} & \multirow{3}{*}{Standard}  & Standard &  \textbf{97.56} \\
                           &                            & Remove Clarifier &  \textbf{97.56} \\
                           &                            & Remove Revert &  \textbf{97.56} \\
                         \cmidrule(lr){2-4}
                           & \multirow{3}{*}{Relaxed}   & Standard & \textbf{98.78} \\
                           &                            & Remove Revert &  98.17 \\
                           &                            & Remove Clarifier &  \textbf{98.78} \\
\bottomrule
\end{tabular}
}
\end{table}


\paragraph{Removing the Clarifier or Revert mechanism.} To see the effect of the Clarifier and Revert mechanism, we remove the two agents from the workflow and measure the workflow pass@1 performance. On HumanEval, we experiment the standard QualityFlow with Code Quality Checker (CQC) and a relaxed QualityFlow with Python checker, presented in Table \ref{tab:removal}. On MBPP, the standard QualityFlow is used. By removing either Clarifier or Revert, we experiment with a total of six ablation settings, and see reduction of pass@1 across all settings, with reduction ranging from 0.78\% to 2.44\% absolutely.




==> 4.discussions.tex <==











==> 5.relatedwork.tex <==
\jason{Need re-write. What is something that existing work cannot do that we can do? Cite fewer papers to avoid steering our reviewers toward certain cohorts that tend to reject our paper. We need to cite more reflection and agentic papers.}

\paragraph{Code LLM}
Large language models (LLMs) have emerged as a powerful tool for various code-related tasks, including program synthesis~\cite{codet5, codet5p, codegen, codegen2, codegeex, incoder, codellama, deepseekcoder, mistral, starcoder2}, bug fixing~\cite{Hossain2024}, program testing~\cite{llm-testing}, and fuzzing~\cite{llm-fuzzing}. These models have exhibited remarkable capabilities in these domains, primarily due to their strong understanding and generation abilities acquired through extensive pre-training on massive datasets. This pre-training enables them to recognize patterns, comprehend context, and generate coherent and contextually relevant code snippets. The impressive performance of LLMs in code-related tasks can be attributed to their ability to learn and capture intricate patterns and relationships from the vast amount of data they are trained on. By exposing these models to a diverse range of code samples, they develop a deep understanding of programming language syntax, semantics, and common coding practices. This knowledge allows them to generate code that adheres to language rules, follows best practices, and aligns with the intended functionality. 
\jason{ Outline our difference.}

\paragraph{Agentic workflow}
Enhancing code generation tasks has become a priority in the field of artificial intelligence, leading to the adoption of AI agentic workflows. These intelligent and autonomous processes leverage multiple AI agents that coordinate a series of operations to accomplish specific objectives or tasks. Notably, MetaGPT\cite{hong2024metagpt} and AgentCoder\cite{agentcoder-self-repair} have embraced this approach to improve their performance. MetaGPT mimics the software development life cycle by employing multiple agents, enabling a more streamlined and efficient process. On the other hand, AgentCoder presents a code generation solution comprising a multi-agent framework that incorporates a specialized test designer agent alongside the traditional program generation and test executor agents. Our proposed QualityFlow distinguishes itself from previous approaches by introducing a quality check agent, which is necessary for control flows in the multi-agent workflow. This addition aims to enhance the overall quality and reliability of the code generation process, ensuring that the generated code meets the desired standards and requirements.
\jason{There can be a ton more papers cited here.}

\paragraph{Self-debug}
Existing techniques have explored using large language models (LLMs) to refine their own generations. Most of these techniques prompt LLMs with execution results~\cite{google-self-debug, mit-self-repair, agentcoder-self-repair, ldb-self-debug, intervenor-chain-of-repair, self-repair-3, self-collaboration, self-repair-2} for refinement. Other approaches involve training LLMs to self-debug. For instance, ILF~\cite{self-repair-1} utilizes human-annotated feedback information, which is not scalable. CYCLE~\cite{cycle-train-self-refine} and Self-Edit~\cite{self-edit}, on the other hand, employ supervised fine-tuning (SFT) to fine-tune LLMs to generate refinements based solely on unit test execution feedback. In contrast, the Self-Debugger agent in this work relies primarily on chain-of-thought prompting, which encourages the LLM to reason about the program's behavior and make informed revisions based on the test cases through a reflective thought process.
\jason{Value?}

\paragraph{Self-reflection} 
Self-reflection is a powerful approach aimed at iteratively enhancing the quality of responses generated by large language models (LLMs). One technique, introduced by Huang et al. (2022) \cite{huang2022large}, employs a pre-trained LLM to generate high-confidence answers, which are subsequently used to fine-tune the same LLM, effectively improving its performance through self-generated solutions. However, the fine-tuning process can be time-consuming and resource-intensive. To address this challenge, Madaan and colleagues \cite{madaan2024self} proposed a novel method called "self-refine," which instructs the LLM to provide feedback on its own output, thereby enabling self-refinement without the need for additional training data or reinforcement learning. Another line of research explores the potential of leveraging multiple LLMs with varying levels of expertise in a collaborative refinement and debating process. Khan et al. \cite{khan2024debating} introduced a framework where two stronger LLMs engage in a debate, presenting arguments and counterarguments, while a weaker model is tasked with evaluating the discussion and selecting the most compelling answer. This approach harnesses the collective knowledge and diverse perspectives of multiple models, potentially leading to more robust and well-reasoned outputs. Our work employs a two-level reflective approach. At the lower level, similar to existing work, we utilize chain-of-thought reflection, which prompts the language model to reason through the problem step-by-step, leading to more logical and coherent revisions. At the higher level, we introduce a Problem Clarifier agent that engages in self-reflection on the entire process flow, allowing it to decide whether to restart the process if necessary. This hierarchical approach combines the benefits of step-by-step reasoning with a higher-level oversight mechanism, aiming to enhance the overall quality and coherence of the generated output.
\jason{Value? Quality Check is the key idea, do we say it or not?}







==> 6.conclusions.tex <==
Deep learning methods have made significant progress in the long-standing problem of program synthesis, and the field has recently been dominated by large language models \cite{codegen, codet5, codellama}. Following the introduction of Generative Pre-training \cite{radford2018improving} and Reinforcement Learning with Human Feedback (RLHF) \cite{ouyang2022training}, improvements in various domains, including program synthesis, have typically come from a small number of research groups with access to a tremendous amount of funding and computation to train large language models.
This approach excludes small, independent researchers from competing or contributing, because their ideas, though valuable and effective as incremental contributions, often cannot directly compare with the state-of-the-art set by the LLMs given limited resources.
It is imperative and a challenge for small independent researchers to effectively integrate their ideas with the LLMs, to improve LLMs' performance without re-training them.
In this context, Agentic Workflows have emerged this year \cite{shinn2024reflexion} and presented much-needed opportunities, thanks to their flexibility to integrate all kinds of subroutines into LLM systems as agents, without re-training the LLMs. Our work is one of the first Agentic Workflow methods to advance this important direction, and we bring the critical component of quality checking to this domain.


Intuitively, it is natural for a well-designed Agentic Workflow to perform better than a single-turn LLM zero-shot synthesis. After all, zero-shot generation with LLMs can be seen as the simplest case of Agentic Workflows that has only one agent.
From this perspective, Agentic Workflows simply allow for more design space than zero-shot generation methods, which should naturally lead to an optimal solution that is at least as good as zero-shot generation, if not better.

Although generic Agentic Workflows such as Reflexion \cite{shinn2024reflexion} and Self-Debate \cite{khan2024debating} may improve program synthesis quality, they ignore lots of opportunities that belong only to the code domain. It is much more interesting to leverage the properties of programs and program execution while designing Agentic Workflows, and existing software engineering (SE) research point to many potential performance improvements. Unlike zero-shot synthesis, where a monolithic LLM produces the solution, Agentic Workflow can include hybrid SE agents that do not rely solely on LLMs. For example, in QualityFlow, we use code execution as an agentic component to provide feedback to the Self-Debugger, and code execution is not an LLM.
Hybrid agents further expands the design space of Agentic Workflows compared to zero-shot LLM synthesis.
An Agentic Workflow can also provide more explainability than a monolithic LLM. One may diagnose specific agents and probe into their performance independently, like our work does for Quality Checkers by measuring their own accuracy, precision, recall, and its effect when included into the workflow.
Hybrid agents and explainability are two desiderata of Agentic Workflows that our work illustrates through QualityFlow as an example.


To leverage code domain properties when designing the Agentic Workflow tailored for program synthesis, our work identifies three important limitations and opportunities: assumption of visible unit test conformity, bottleneck of synthesized test quality, and deviation of self-debugging trajectory. The three limitations are tackled by one carefully designed controller agentic, the Quality Checker, which examines visible test conformity, rejects potentially incorrect programs from self-debugging due to incorrect tests, and navigates the dynamic workflow by restarting or resetting potentially deviated trajectories. Our Quality Checker uses Imagined Execution and is highly accurate in making these decisions. Perhaps for program synthesis, what matters is not to produce the correct solution somewhere in the workflow, but rather to identify the correct solution and capture it as the final answer. This is the key perspective from the Quality Checker, which is carried further by Diversified Prompting. As a result, QualityFlow establishes the new state-of-the-art results on four benchmarks: MBPP, HumanEval, and EvalPlus evaluations for both.

Through comprehensive analysis, QualityFlow shows consistent performance improvements over zero-shot generation under different settings. QualityFlow's performance generalizes over different LLM backbones, which allows QualityFlow to grow naturally when better LLMs are trained in the future and used in QualityFlow. The research efforts on Agentic Workflows and LLMs are not competitive against each other, but rather orthogonal and symbiotic.


Agentic Workflows is developing quickly into a major artificial intelligence paradigm with emerging applications including software development \cite{amazonAssistantAmazon}. 
In future work, one possible research direction is to further develop the Test Quality Checker, as the bottleneck of synthesized test quality is a relatively more challenging problem that is mitigated but not completely addressed by our TQC.
More generally, the idea of quality checks and diversified prompting could easily be applied to other problem domains to create dynamic workflows and navigate them. 
Agentic Workflows provide fertile opportunities to build the next generation of AI systems powered by large language models, and we invite the community to conduct further research.


























\section{\jason{Work in progress}}


Need to highlight interesting ideas and impact on the field. The writing is limited to facts only and too dry. More value statements are needed.
What is the idea that is explored? Not the task executed, but the idea behind, and why the idea itself is interesting/impactful. The idea is the purpose.

Models that run on MBXP (cited Athi paper).
\begin{enumerate}
    \item https://dl.acm.org/doi/pdf/10.1145/3690635 MBCPP
    \item https://dl.acm.org/doi/pdf/10.1145/3675395 
    \item https://arxiv.org/pdf/2310.09748 MBJP, MBCPP
    \item https://dl.acm.org/doi/pdf/10.1145/3675395 PP, JP, JSP
    \item https://arxiv.org/pdf/2303.17780 PP, JP, JSP
\end{enumerate}


Token count.

Add symbols to the methods for ICML taste, problem definition at the beginning of methods.

Figure 2 needs to be more professional. The coloring is not good.

Related work needs to raise the bar.

Throughout the paper, factual statements are not only correct, but also need to deliver an interesting/impactful argument, or serve as reasons for an impactful conclusion and connect.




==> backup.tex <==


























































==> introduction.tex <==
Large Language Models (LLMs) have demonstrated significant advancements in various code-related tasks, particularly in code generation, where they synthesize source code from natural language problem descriptions \cite{mbpp, humaneval, apps}. 
\jason{Code generation is an impactful problem that could enable}
As LLM methods for code generation continue to evolve, approaches have progressed from the initial zero-shot generation to more sophisticated techniques like self-debugging and Reflexion \cite{}, leading to increasingly improved performance. In zero-shot generation, a single call to the LLM is made, relying solely on the capabilities of the pre-trained model for code generation. Most modern foundational models are pre-trained on code-related tasks, making this approach effective. In contrast, self-debugging involves executing unit tests associated with the problem statement. By running the synthesized code, identifying failed cases, and incorporating error and trace information, a richer prompt is created to query the LLM, allowing it to revise the code with the goal of passing the previously failed tests.


Code generation is a prominent problem that attracts attention.


In recent years, generations of ML solutions have been introduced to advance the performance of machine learning code generation (relevant, and set a low baseline). 
Seq2Seq translations, fine-tuning pre-trained models solution, instruction LLMs, multi-LLM methods (Reflexion). 
ABCDE.
What will be the next pocket of opportunities and improvements for code generation models?

In our view, there are a few questions that existing work ignored to address, inviting opportunities.
ABCDE.

We propose QualityFlow, ... 

To summarize,

\jason{Introduction: demonstrate novelty.}


\jason{We should compare with older state of the art methods. FSE is not as fast as ML venues. }

There are several major issues with the existing LLM methods for code generation.
1. decision-making through agentic workflow.
2. During self-debugging, the usage of visible unit tests are too naive. For datasets with separated of visible and hidden unit tests, e.g., HumanEval, the visible test samples are typically simply executed to gather error or trace information. However, for some samples in the dataset, the provided visible tests are too simple and easy to pass but usually the generated program will fail in executing the hidden tests. While for dataset like MBPP as there are no hidden tests, part of the tests are treated as visible and executed to participate in the self-debugging, which violates the pass@1 requirement. The option of emulating the process of execution of the tests without actually running them which could potentially provide better context for self-debugging hasn't been explored. Second, the quality of the test generator could become the bottleneck of the entire system. Incorrect tests could easily push the self-debugger make wrong revisions on the code, in its worst case, it make the originally correct code goes wrong. Third, it lacks an effective hard reset mechanism that could be effectively when the initially generated code is very wrong. Mis-understanding the problem description often happens to human developer and also observed in LLMs, with a largely wrong code to start with, even lots of efforts are spent on test generation and self-debugging it might not be able to reach a correct answer. A reset and re-try mechanism should be considered in such situations.  

\jason{Three selling points that existing work does not have: decision-making through agentic workflow. code-specific critiques. }


In this paper, we propose an innovative multi-agent based code generation solution which integrates the ideas of chain-of-thought based code/test quality checker, test synthesis, self debugging and problem clarifier. The agentic flow consists 8 agents working together to generate code, synthesize unit tests, perform self debugging, conduct quality check and re-phrase the problem statement. One of the main innovation besides the proposed agentic flow is the quality checker, it could emulate the problem execution process without actually execute the code based on step-by-step reasoning. This module is essential for generate pass@1 solution for dataset without separation of visible and hidden tests such as MBPP, and it also helps in case of the visible tests are easy to pass but the hidden tests are more challenging. Another contribution is the introduction of the clarifier, the purpose of this agent is to re-paraphrase the problem statement given the context of repeated failures in self-debugging which raises reasonable doubts that the initially generated program might misunderstood the problem statement and the program is totally wrong and beyond repair with self-debugging and thus synthesize the new program given all these context could be a better choice.


==> macros.tex <==


\newcommand{\todoc}[2]{{\textcolor{#1}{#2}}}
\newcommand{\todoblack}[1]{{\todoc{black}{\textbf{[[#1]]}}}}
\newcommand{\todored}[1]{{\todoc{red}{\textbf{[[#1]]}}}}
\newcommand{\todogreen}[1]{\todoc{green}{\textbf{[[#1]]}}}
\newcommand{\todoblue}[1]{\todoc{black}{#1}}
\newcommand{\todoorange}[1]{\todoc{orange}{\textbf{[[#1]]}}}
\newcommand{\todobrown}[1]{\todoc{brown}{\textbf{[[#1]]}}}
\newcommand{\todogray}[1]{\todoc{gray}{\textbf{[[#1]]}}}
\newcommand{\todopurple}[1]{\todoc{purple}{\textbf{[[#1]]}}}
\newcommand{\todopink}[1]{\todoc{magenta}{\textbf{[[#1]]}}}
\newcommand{\todocyan}[1]{\todoc{cyan}{\textbf{[[#1]]}}}
\newcommand{\todoviolet}[1]{\todoc{violet}{\textbf{[[#1]]}}}
\newcommand{\todo}[1]{\todored{TODO: #1}}


\newcommand{\nan}[1]{\todopink{Nan: #1}}
\newcommand{\soneya}[1]{\todogreen{Soneya: #1}}
\newcommand{\qiang}[1]{\todoorange{Qiang: #1}}
\newcommand{\mr}[1]{\todoblue{#1}}
\newcommand{\toolname}{Toggle}




\newcommand{\code}[1]{\texttt{\small #1}} %

\newcounter{finding}
\newcommand{\finding}[1]{\refstepcounter{finding}
    \begin{mdframed}[linecolor=gray,roundcorner=12pt,backgroundcolor=gray!15,linewidth=3pt,innerleftmargin=2pt, leftmargin=0cm,rightmargin=0cm,topline=false,bottomline=false,rightline=false]
        \textbf{Finding \arabic{finding}:} #1
    \end{mdframed}
}

